Towards PAC Multi-Object Detection and Tracking

Accurately detecting and tracking multi-objects is important for safety-critical applications such as autonomous navigation. However, it remains challenging to provide guarantees on the performance of state-of-the-art techniques based on deep learning. We consider a strategy known as conformal prediction, which predicts sets of labels instead of a single label; in the classification and regression settings, these algorithms can guarantee that the true label lies within the prediction set with high probability. Building on these ideas, we propose multi-object detection and tracking algorithms that come with probably approximately correct (PAC) guarantees. They do so by constructing both a prediction set around each object detection as well as around the set of edge transitions; given an object, the detection prediction set contains its true bounding box with high probability, and the edge prediction set contains its true transition across frames with high probability. We empirically demonstrate that our method can detect and track objects with PAC guarantees on the COCO and MOT-17 datasets.

==> figs/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\columnwidth]{example-image-golden}
\hfill
\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Outline -- }
A figure summarizing the entire algorithm
}
\label{fig:overview}
\end{figure*}

==> figs/teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Teaser -- }
Some nice summarizing image.
}
\label{fig:teaser}
\end{figure}

==> sec/1_introduction.tex <==
%% !TEX root = ../pac_det_mot.tex

\section{Introduction}

%% motivation:  detection + tracking used in safety critical systems need to be correct
Visual multi-object detectors and trackers are essential parts for vision-based autonomous systems \citep{TODO}, which have been actively researched for decades \citep{}. As they are deployed in safety critical systems, understanding the correctness on the detection and tracking uncertainty predictions needs to be considered, but it was under-explored so far, possibly resulting in life-threatening accidents.
%---\eg the death of Elaine Herzberg by a Uber self-driving car.

%% motivation: uncertainty quantification is required on complex systems, e.g., detectors or trackers
Uncertainty quantification \citep{TODO} has received more attention as deep neural networks gets deployed in real world systems \citep{TODO}.
In particular, prediction sets provide uncertainty over label predictions, which come with theoretical guarantees \citep{TODO} for classification and regression. However, detections and tracking require more complex predictors, rather than a single classifier or regressor, which poses challenges to applying the existing prediction set approaches directly to detections and tracking. 

%% our approach
In this paper, we propose novel compositional approaches to provide the correct guarantee for multi-object detectors and trackers. In particular, we use PAC prediction sets \citep{Park2020PAC} as a building block, and provide a PAC guarantee for the \emph{entire} detectors and trackers based on PAC guarantees for the \emph{individual} components. 
%% approach details: detection
For detection, we take faster RCNN detector \citep{Ren2015FasterRT} as an example; it consists of three components: proposal, presence, and location components. The proposal component provides bounding boxes, or proposals,  over an image which likely contains objects. The presence component outputs the likelihood of the presence of a target object class in the proposals from the proposal component. Similarly, the location component outputs the location of the target object class in the proposals. Finally, the detector returns a set of the presence and location pair for final detection outputs. In this use case, we apply the PAC prediction set approach for individual components to make individual PAC guarantees, with which we can prove that the composed detector also satisfies a PAC guarantee. 

%% approach details: tracking
For tracking, we build on Trackor \citep{Bergmann_2019}, which is composed of an object detection component and an object connection component. The object detection component outputs the pair of an object presence score and object location for each image, which can be obtained by running an off-the-shelf object detector. The object connection component predicts the connection, or \emph{edge}, between pairs object detections at the adjacent time frames based on their similarities---\eg location similarity from the intersection over union (IoU) between two bounding boxes, object class similarity between a per-image predicted class via object detection, and an inter-image predicted class via a Hidden Markov Model (HMM). Here, we provide the PAC guarantee for the edge predictions for one-step multi-object tracking. 


%% results summary
\SP{add results summary}

In the tracking problem, our edge prediction sets are $(\epsilon, \delta)$-correct, satisfying the required error and confidence level. Comparing to other baselines, our edge prediction sets achieve lower false positive rate while satisfying the false negative rate constraint. 





==> sec/2_related.tex <==
%% !TEX root = ../pac_det_mot.tex


%%
%% related work
%%
\section{Related Work}
\subsection{Detection}
\textbf{One-stage detector}
Conventional one-stage detectors typically use a straightforward fully convolutional design, with the network's outputs being classification probabilities and box offsets (w.r.t. a pre-defined target bounding box) for each spatial location.
For example, YOLO \cite{Redmon2016YouOL} is the first attempt at creating a real-time object detector that is fast. Since YOLO skips the area proposal stage and only predicts over a small number of bounding boxes, it can perform inference extremely quickly. Unlike YOLO, Single Shot Detector (SSD) \cite{Liu2016SSDSS} predicts the offset of predefined anchor boxes (referred to as \emph{default boxes} in their paper) for each position of the function diagram, rather than splitting the image into grids of arbitrary dimension. SSD encapsulates all processing in a single network as well, which prevents proposal generation and subsequent pixel or feature resampling.  Each box has a fixed size and location in relation to the cell it belongs to. Per function map location, SSD discretizes the output space of bounding boxes into a collection of default boxes at various aspect ratios and sizes. The network creates scores for the existence of each object category in each default box at prediction time, and then adjusts the box to best match the object shape.


\textbf{Two-stage detector}
% (Mask-RCNN:https://arxiv.org/pdf/1703.06870.pdf, Faster-RCNN: https://arxiv.org/pdf/1506.01497.pdf, Fast-RCNN: https://arxiv.org/pdf/1504.08083.pdf)
Two-stage detectors, on the other hand, have a more complex pipeline. They first use an area proposal network (RPN) to screen out the regions in the picture that have a high chance of containing an object.
The proposals are then fed into the region convolutional network (R-CNN) \cite{He2017MaskR} to obtain their classification score and spatial offsets. While one-stage detectors are more simple in architecture, two-stage detectors currently dominate in accuracy. Training an R-CNN model is expensive and slow, owing to the sequential process of selective search and feature generation.
Girshick introduced Fast R-CNN \cite{Girshick2015FastR} to optimize RCNN-training procedure by combining three separate models into a single jointly qualified system and increasing mutual calculation performance. Rather than extracting CNN feature vectors for each region proposal separately, this model combines them into a single CNN forward pass over the entire image, and the region proposals share this feature matrix. The same function matrix is then split up and used to train the object classifier and bounding-box regressor.
Faster R-CNN advanced the computation speed of Fast R-CNN by integrating the region proposal algorithm into the CNN model. They introduce a Region Proposal Network (RPN) that shares full-image convolutional features with the detection network, allowing region proposals to be made for almost no computational cost. 
Faster R-CNN \cite{Ren2015FasterRT} is later extended by Mask R-CNN, which adds a branch for predicting an object mask to the current branch for bounding box recognition. Mask R-CNN is easy to train and introduces a slight amount of overhead to Faster R-CNN.



\textbf{Proposed set-based and Probabilistic Object Detector}
Apart from the above two classic categories, there are some recently emerged object detectors. For instance, DETR \cite{carion2020end} treats the object detection problem to be a direct set prediction problem. It uses a set-based global loss that forces unique predictions via bipartite matching, and a transformer encoder-decoder architecture. The probabilistic object detector extends standard object detectors and estimates predictive distributions for output categories and bounding boxes simultaneously. For example, the work \cite{harakeh2021estimating} extends one-stage (RetinaNet), two-stage (FasterRCNN), and the proposed set-based (DETR) object detectors to output a distribution over bounding box regression output with variance networks. 

% \SP{probabilistic object detector (https://arxiv.org/pdf/2101.05036.pdf): they extends detectron2 to output a distribution over bounding boxes; check references in this paper.}

\subsection{Tracking}
Many safety-critical tasks involve tracking multi-objects. However, multi-object tracking still remains a challenge problem despite current advancement in deep learning \cite{luo2017multiple}. Most multi-object tracking algorithms employ the \textit{Tracking-by-detection} paradigm \cite{10.1007/978-3-319-11752-2_21, 10.1007/978-3-642-33709-3_25, article}. This paradigm consists of two steps, namely individual object localization in each frame and track formation by associating object detection across time steps. 

The object detection step is often tackled by object detectors like Faster-RCNN \cite{he2016deep} or SDP \cite{7780603}. The data association problem is often represented as a graph, where detected objects are nodes and link between detected objects are edges. This problem could be attacked by a frame-by-frame\cite{5459278, 4587581, 20.500.11850/156675} or track-by-track scheme \cite{article}. 

In order to improve the tracking performance, many algorithms utilize Kalman Filter \cite{Li2010AMO, 6935235, 5512258}. For the motion model, some papers make the constant velocity assumption\cite{5995311, 10.1007/978-3-642-15561-1_40}, while others turn to more expressive models like Social Force Model\cite{5995468, 6130233, inproceeding}. Furthermore, some papers utilize deep learning to extract motion models in crowded scenarios \cite{7780479, inproceedingss}. Objection detection results could be regarded as measurements in Kalman Filter. The measurement uncertainty could either be assigned a constant value or estimated at each time step by the detector.

Furthermore, for the re-identification step in multi-object tracking problem, many papers rely on color-based models\cite{article2}. However, these methods may fell short when pedestrians wear similar clothes.

In this paper, we build on the work of Tracktor \cite{Bergmann_2019}. It only relies on an object detection algorithm to attack tracking problem. Specifically, Tracktor utilizes the regression head of a detector to realign object object bounding boxes; it then utilizes a Siamese network to accomplish re-identification.




\subsection{Uncertainty Quantification}
\SP{add this}


\SP{remind the application to single object tracking}



==> sec/3_method.tex <==
\section{Method}
\lorem{1}



==> sec/4_results.tex <==
\input{tab/sota}
\input{tab/ablations}

\section{Results}
See \Table{sota} and \Table{ablations}.
\lorem{5}


==> sec/5_conclusions.tex <==
\section{Conclusions}
\lorem{3}


==> sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/header.tex <==
% Jim's packages and definitions. Modified by Sangdon

%%
%% packages 
%%
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{tikz} % tikz for graphics drawing
%\usepackage{pgfplots} % tikz axis
%\usepackage{algorithm}% http://ctan.org/pkg/algorithms
%\usepackage{algorithmicx}
%\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx
%\usepackage{romannum} % Romman numbers
%\usepackage{multirow} % multirow in tables
%\usepackage{cprotect} % when add citations in captions
%\usepackage{stackrel}% http://ctan.org/pkg/stackrel
\usepackage{amsmath} % http://ctan.org/pkg/amsmath
%\usepackage{amsfonts} % http://ctan.org/pkg/amsfonts
\usepackage{bm} % for bold symbols like \bm{\alpha} or {\bm \alpha\beta}
\usepackage{bbm} % for mathbbm
%\usepackage{MnSymbol} % double angle brackets...
%\usepackage{mathtools} % for 
%\usepackage{diagbox} % \diagbox[]{}{}
%\usepackage{tabulary} % \newcolumntype
%\usepackage{rotating} % vertical table       
%\usepackage{subcaption} % subfigure
%\usepackage{graphicx}
%\usepackage{gensymb}
%\usepackage{color}
%\usepackage{subfig}
%\usepackage{textcomp}
%\usepackage{amssymb}
%%\usepackage{multicol, multirow}
%\usepackage{amsthm}
%%\usepackage{arydshln}
%%\usepackage{mathtools}
%\usepackage{makecell}
%
%
%
%\usepackage{subfloat}
%\usepackage{caption}
%
%
%
%\graphicspath{{figs/}}
%\usepackage{paralist}
%
%
%
%
%\usepackage{bm} % for bold symbols like \bm{\alpha} or {\bm \alpha\beta}
%
%%																	%
%\usepackage{balance}
%\usepackage{comment}
%\usepackage{psfrag}
%
%\usepackage{enumerate}
%\usepackage{epsfig}
%\usepackage{setspace}
%
%\usepackage{epstopdf} % Jose loves this
%
%
%\newcommand{\reviewnote}[3]{#1\footnote{\textcolor{red}{#2: #3}}}
%
%% Clever references -- SHOULD BE LOADED LAST
%% Generic commands: \cref and \Cref
%% Seems incompatible with `algorithmic' from algorithms bundle, but can be used with `algorithmicx' (e.g. `algpseudocode').
%\usepackage[capitalise]{cleveref}
%\newcommand{\vref}[1]{\cref{#1}}
%% When using \namecref, cleveref capitalizes the first character if the option capitalise is used, which I don't want.  So use \lcnamecref instead.
%
%
%


%%
%% beamer
%%
%%\usepackage{appendixnumberbeamer}      
%\usepackage{pifont}% http://ctan.org/pkg/pifont
%\newcommand{\cmark}{{\color{ForestGreen}\ding{51}}} % check mark
%\newcommand{\xmark}{{\color{red}\ding{55}}} % x mark


\makeatletter
\@ifundefined{proposition}{%
    \newtheorem{proposition}{Proposition}
}{}
%\@ifundefined{proposition*}{%
%    \newtheorem*{proposition*}{Proposition}
%}{}
\@ifundefined{definition}{%
    \newtheorem{definition}{Definition}%
}{}
\@ifundefined{lemma}{%
    \newtheorem{lemma}{Lemma}
}{}
%\@ifundefined{lemma*}{%
%\newtheorem*{lemma*}{Lemma}
%}{}
\@ifundefined{corollary}{%
    \newtheorem{corollary}{Corollary}
}{}
\@ifundefined{theorem}{%
    \newtheorem{theorem}{Theorem}
}{}
%\@ifundefined{theorem*}{%
%    \newtheorem*{theorem*}{Theorem}
%}{}
\@ifundefined{corollary}{%
    \newtheorem{corollary}{Corollary}
}{}
%\@ifundefined{corollary*}{%
%    \newtheorem*{corollary*}{Corollary}
%}{}
\@ifundefined{assumption}{%
    \newtheorem{assumption}{Assumption}
}{}
\@ifundefined{problem}{%
    \newtheorem{problem}{Problem}
}{}
%\@ifundefined{problem*}{%
%    \newtheorem*{problem*}{Problem}
%}{}
\@ifundefined{claim}{%
    \newtheorem{claim}{claim}
}{}
\makeatother

\newtheorem{innercustomthm}{Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

\newtheorem{innercustomprop}{Proposition}
\newenvironment{customprop}[1]
  {\renewcommand\theinnercustomprop{#1}\innercustomprop}
  {\endinnercustomprop}

\newtheorem{innercustomcor}{Corollary}
\newenvironment{customcor}[1]
  {\renewcommand\theinnercustomcor{#1}\innercustomcor}
  {\endinnercustomcor}

\newtheorem{innercustomlem}{Lemma}
\newenvironment{customlem}[1]
  {\renewcommand\theinnercustomlem{#1}\innercustomlem}
  {\endinnercustomlem}


%%
%% Definitions
%%


%%% tikz
%\usetikzlibrary{matrix} % for block alignment
%\usetikzlibrary{arrows} % for arrow heads
%\usetikzlibrary{calc} % for manimulation of coordinates
%\usetikzlibrary{fit,positioning, shapes.misc, backgrounds}
%\usetikzlibrary{patterns}

%% algorithm
\let\oldReturn\Return
%\renewcommand{\Return}{\State\oldReturn}
\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\Break}{\STATE \algorithmicbreak}
%\algdef{SE}[DOWHILE]{Do}{DoWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}

%% math
%% \DeclareMathOperator{\sech}{sech}
%%\DeclareMathOperator{\sign}{sign}
%% \DeclareMathOperator{\diag}{diag}

%% theorem-like paragraphes
%\newtheorem{definition}{Definition} % add [section]
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{proposition}{Proposition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{claim}{Claim}
%\newtheorem{problem}{Problem}

% custom theorem
\newtheorem{innercustomgeneric}{\customgenericname}
\providecommand{\customgenericname}{}
\newcommand{\newcustomtheorem}[2]{%
  \newenvironment{#1}[1]
  {%
   \renewcommand\customgenericname{#2}%
   \renewcommand\theinnercustomgeneric{##1}%
   \innercustomgeneric
  }
  {\endinnercustomgeneric}
}
\newcustomtheorem{customclaim}{Claim}

%\newtheorem*{problem*}{Problem}
%\newtheorem*{definition*}{Definition}

%% shorthands for references
\providecommand{\Fig}{Figure~}
\providecommand{\Sec}{Section~}
\providecommand{\Tab}{Table~}
\providecommand{\Alg}{Algorithm~}
\providecommand{\Eq}{Equation~}
\providecommand{\Def}{Definition~}
\providecommand{\Thm}{Theorem~}
\providecommand{\Pro}{Proposition~}
\providecommand{\Lem}{Lemma~}

%% shorthands for labels, equations, matrices...
\providecommand{\eqnref}			[1]		{Equation~(\ref{#1})}
\providecommand{\tabref}			[1]		{Table~\ref{#1}}
\providecommand{\figref}			[1]		{Figure~\ref{#1}}
\providecommand{\alref}			[1]		{Algorithm~\ref{#1}}
\providecommand{\defref}			[1]		{Definition~\ref{#1}}
\providecommand{\prbref}			[1]		{Problem~\ref{#1}}
\providecommand{\thmref}			[1]		{Theorem~\ref{#1}}
\providecommand{\proref}			[1]		{Proposition~\ref{#1}}
\providecommand{\lemref}			[1]		{Lemma~\ref{#1}}
\providecommand{\corref}			[1]		{Corollary~\ref{#1}}
\providecommand{\secref}			[1]		{Section~\ref{#1}}
\providecommand{\apxref}			[1]		{Appendix~\ref{#1}}

\providecommand{\eqa}				[1]		{\begin{align}#1\end{align}}
\providecommand{\eqas}			[1]		{\begin{align*}#1\end{align*}}
\providecommand{\eqml}			[1]		{\begin{multline}#1\end{multline}}
\providecommand{\mat}				[2]		{\left[\begin{array}{#1} #2 \end{array}\right]}

%% shorthands for abbreviations for Latin terms.
\providecommand{\ie}{\emph{i.e.,}~}
\providecommand{\eg}{\emph{e.g.,}~}

%% aux
\providecommand\qcomment[1]{ }

%% Number types
\providecommand{\realnum}					{\mathbb{R}}
\providecommand{\integernum}				{\mathbb{Z}}
\providecommand{\complexnum}				{\mathbb{C}}
\providecommand{\naturalnum}				{\mathbb{N}}

%% Common mathematical functions and symbols
\renewcommand{\(}						{\left(}
\renewcommand{\)}						{\right)}
\renewcommand{\[}						{\left[}
\renewcommand{\]}						{\right]}
\newcommand{\<}						{\left<}
\renewcommand{\>}						{\right>}

%% shorthands for useful functions, expectation, probability, indicator function
\providecommand{\Prob}{\mathbbm{P}}
\providecommand{\Probop}{\mathop{\Prob}}
\providecommand{\Exp}{\mathbbm{E}}
\providecommand{\Expop}{\mathop{\Exp}}
\providecommand{\Ind}{\mathbbm{I}}
\providecommand{\iid}{i.i.d.}
\providecommand{\findop}{\mathop{\text{find}}}

%% Jim's alphabet definitions

%% bold lower case
\def\a{\bm{a}}
\def\b{\bm{b}}
\def\c{\bm{c}}
\def\d{\bm{d}}
\def\e{\bm{e}}
\def\f{\bm{f}}
\def\g{\bm{g}}
\def\h{\bm{h}}
\def\i{\bm{i}}
\def\i{\bm{j}}
\def\k{\bm{k}}
\def\l{\bm{l}}
\def\m{\bm{m}}
\def\n{\bm{n}}
%\def\o{\bm{o}}
\def\p{\bm{p}}
\def\q{\bm{q}}
\def\r{\bm{r}}
\def\s{\bm{s}}
\def\t{\bm{t}}
\def\u{\bm{u}}
\def\v{\bm{v}}
\def\w{\bm{w}}
\def\x{\bm{x}}
\def\y{\bm{y}}
\def\z{\bm{z}}
\def\A{\bm{A}}
\def\B{\bm{B}}
\def\C{\bm{C}}
\def\D{\bm{D}}
\def\E{\bm{E}}
\def\F{\bm{F}}
\def\G{\bm{G}}
\def\H{\bm{H}}
\def\I{\bm{I}}
\def\J{\bm{J}}
\def\K{\bm{K}}
\def\L{\bm{L}}
\def\M{\bm{M}}
\def\N{\bm{N}}
\def\O{\bm{O}}
\def\P{\bm{P}}
\def\Q{\bm{Q}}
\def\R{\bm{R}}
\def\S{\bm{S}}
\def\T{\bm{T}}
\def\U{\bm{U}}
\def\V{\bm{V}}
\def\W{\bm{W}}
\def\X{\bm{X}}
\def\Y{\bm{Y}}
\def\Z{\bm{Z}}
%
%
%
%% bold hat
\def\aH{\hat{\bm{a}}}
\def\bH{\hat{\bm{b}}}
\def\cH{\hat{\bm{c}}}
\def\dH{\hat{\bm{d}}}
\def\eH{\hat{\bm{e}}}
\def\fH{\hat{\bm{f}}}
\def\gH{\hat{\bm{g}}}
\def\hH{\hat{\bm{h}}}
\def\iH{\hat{\bm{i}}}
\def\iH{\hat{\bm{j}}}
\def\kH{\hat{\bm{k}}}
\def\lH{\hat{\bm{l}}}
\def\mH{\hat{\bm{m}}}
\def\nH{\hat{\bm{n}}}
\def\oH{\hat{\bm{o}}}
\def\pH{\hat{\bm{p}}}
\def\qH{\hat{\bm{q}}}
\def\rH{\hat{\bm{r}}}
\def\sH{\hat{\bm{s}}}
\def\tH{\hat{\bm{t}}}
\def\uH{\hat{\bm{u}}}
\def\vH{\hat{\bm{v}}}
\def\wH{\hat{\bm{w}}}
\def\xH{\hat{\bm{x}}}
\def\yH{\hat{\bm{y}}}
\def\zH{\hat{\bm{z}}}
\def\AH{\hat{\bm{A}}}
\def\BH{\hat{\bm{B}}}
\def\CH{\hat{\bm{C}}}
\def\DH{\hat{\bm{D}}}
\def\EH{\hat{\bm{E}}}
\def\FH{\hat{\bm{F}}}
\def\GH{\hat{\bm{G}}}
\def\HH{\hat{\bm{H}}}
\def\IH{\hat{\bm{I}}}
\def\JH{\hat{\bm{J}}}
\def\KH{\hat{\bm{K}}}
\def\LH{\hat{\bm{L}}}
\def\MH{\hat{\bm{M}}}
\def\NH{\hat{\bm{N}}}
\def\OH{\hat{\bm{O}}}
\def\PH{\hat{\bm{P}}}
\def\QH{\hat{\bm{Q}}}
\def\RH{\hat{\bm{R}}}
\def\SH{\hat{\bm{S}}}
\def\TH{\hat{\bm{T}}}
\def\UH{\hat{\bm{U}}}
\def\VH{\hat{\bm{V}}}
\def\WH{\hat{\bm{W}}}
\def\XH{\hat{\bm{X}}}
\def\YH{\hat{\bm{Y}}}
\def\ZH{\hat{\bm{Z}}}
%
% bold bar
\def\aB{\bar{\bm{a}}}
\def\bB{\bar{\bm{b}}}
\def\cB{\bar{\bm{c}}}
\def\dB{\bar{\bm{d}}}
\def\eB{\bar{\bm{e}}}
\def\fB{\bar{\bm{f}}}
\def\gB{\bar{\bm{g}}}
\def\hB{\bar{\bm{h}}}
\def\iB{\bar{\bm{i}}}
\def\iB{\bar{\bm{j}}}
\def\kB{\bar{\bm{k}}}
\def\lB{\bar{\bm{l}}}
\def\mB{\bar{\bm{m}}}
\def\nB{\bar{\bm{n}}}
\def\oB{\bar{\bm{o}}}
\def\pB{\bar{\bm{p}}}
\def\qB{\bar{\bm{q}}}
\def\rB{\bar{\bm{r}}}
\def\sB{\bar{\bm{s}}}
\def\tB{\bar{\bm{t}}}
\def\uB{\bar{\bm{u}}}
\def\vB{\bar{\bm{v}}}
\def\wB{\bar{\bm{w}}}
\def\xB{\bar{\bm{x}}}
\def\yB{\bar{\bm{y}}}
\def\zB{\bar{\bm{z}}}
\def\AB{\bar{\bm{A}}}
\def\BB{\bar{\bm{B}}}
\def\CB{\bar{\bm{C}}}
\def\DB{\bar{\bm{D}}}
\def\EB{\bar{\bm{E}}}
\def\FB{\bar{\bm{F}}}
\def\GB{\bar{\bm{G}}}
\def\HB{\bar{\bm{H}}}
\def\IB{\bar{\bm{I}}}
\def\JB{\bar{\bm{J}}}
\def\KB{\bar{\bm{K}}}
\def\LB{\bar{\bm{L}}}
\def\MB{\bar{\bm{M}}}
\def\NB{\bar{\bm{N}}}
\def\OB{\bar{\bm{O}}}
\def\PB{\bar{\bm{P}}}
\def\QB{\bar{\bm{Q}}}
\def\RB{\bar{\bm{R}}}
\def\SB{\bar{\bm{S}}}
\def\TB{\bar{\bm{T}}}
\def\UB{\bar{\bm{U}}}
\def\VB{\bar{\bm{V}}}
\def\WB{\bar{\bm{W}}}
\def\XB{\bar{\bm{X}}}
\def\YB{\bar{\bm{Y}}}
\def\ZB{\bar{\bm{Z}}}
%
%%% bold tilde
%%\def\aT{\tilde{\bm{a}}}
%%\def\bT{\tilde{\bm{b}}}
%%\def\cT{\tilde{\bm{c}}}
%%\def\dT{\tilde{\bm{d}}}
%%\def\eT{\tilde{\bm{e}}}
%%\def\fT{\tilde{\bm{f}}}
%%\def\gT{\tilde{\bm{g}}}
%%\def\hT{\tilde{\bm{h}}}
%%\def\iT{\tilde{\bm{i}}}
%%\def\iT{\tilde{\bm{j}}}
%%\def\kT{\tilde{\bm{k}}}
%%\def\lT{\tilde{\bm{l}}}
%%\def\mT{\tilde{\bm{m}}}
%%\def\nT{\tilde{\bm{n}}}
%%\def\oT{\tilde{\bm{o}}}
%%\def\pT{\tilde{\bm{p}}}
%%\def\qT{\tilde{\bm{q}}}
%%\def\rT{\tilde{\bm{r}}}
%%\def\sT{\tilde{\bm{s}}}
%%\def\tT{\tilde{\bm{t}}}
%%\def\uT{\tilde{\bm{u}}}
%%\def\vT{\tilde{\bm{v}}}
%%\def\wT{\tilde{\bm{w}}}
%%\def\xT{\tilde{\bm{x}}}
%%\def\yT{\tilde{\bm{y}}}
%%\def\zT{\tilde{\bm{z}}}
%%\def\AT{\tilde{\bm{A}}}
%%\def\BT{\tilde{\bm{B}}}
%%\def\CT{\tilde{\bm{C}}}
%%\def\DT{\tilde{\bm{D}}}
%%\def\ET{\tilde{\bm{E}}}
%%\def\FT{\tilde{\bm{F}}}
%%\def\GT{\tilde{\bm{G}}}
%%\def\HT{\tilde{\bm{H}}}
%%\def\IT{\tilde{\bm{I}}}
%%\def\JT{\tilde{\bm{J}}}
%%\def\KT{\tilde{\bm{K}}}
%%\def\LT{\tilde{\bm{L}}}
%%\def\MT{\tilde{\bm{M}}}
%%\def\NT{\tilde{\bm{N}}}
%%\def\OT{\tilde{\bm{O}}}
%%\def\PT{\tilde{\bm{P}}}
%%\def\QT{\tilde{\bm{Q}}}
%%\def\RT{\tilde{\bm{R}}}
%%\def\ST{\tilde{\bm{S}}}
%%\def\TT{\tilde{\bm{T}}}
%%\def\UT{\tilde{\bm{U}}}
%%\def\VT{\tilde{\bm{V}}}
%%\def\WT{\tilde{\bm{W}}}
%%\def\XT{\tilde{\bm{X}}}
%%\def\YT{\tilde{\bm{Y}}}
%%\def\ZT{\tilde{\bm{Z}}}
%
%% bold vec
%\def\aV{\vec{\bm{a}}}
%\def\bV{\vec{\bm{b}}}
%\def\cV{\vec{\bm{c}}}
%\def\dV{\vec{\bm{d}}}
%\def\eV{\vec{\bm{e}}}
%\def\fV{\vec{\bm{f}}}
%\def\gV{\vec{\bm{g}}}
%\def\hV{\vec{\bm{h}}}
%\def\iV{\vec{\bm{i}}}
%\def\iV{\vec{\bm{j}}}
%\def\kV{\vec{\bm{k}}}
%\def\lV{\vec{\bm{l}}}
%\def\mV{\vec{\bm{m}}}
%\def\nV{\vec{\bm{n}}}
%\def\oV{\vec{\bm{o}}}
%\def\pV{\vec{\bm{p}}}
%\def\qV{\vec{\bm{q}}}
%\def\rV{\vec{\bm{r}}}
%\def\sV{\vec{\bm{s}}}
%\def\tV{\vec{\bm{t}}}
%\def\uV{\vec{\bm{u}}}
%\def\vV{\vec{\bm{v}}}
%\def\wV{\vec{\bm{w}}}
%\def\xV{\vec{\bm{x}}}
%\def\yV{\vec{\bm{y}}}
%\def\zV{\vec{\bm{z}}}
%\def\AV{\vec{\bm{A}}}
%\def\BV{\vec{\bm{B}}}
%\def\CV{\vec{\bm{C}}}
%\def\DV{\vec{\bm{D}}}
%\def\EV{\vec{\bm{E}}}
%\def\FV{\vec{\bm{F}}}
%\def\GV{\vec{\bm{G}}}
%\def\HV{\vec{\bm{H}}}
%\def\IV{\vec{\bm{I}}}
%\def\JV{\vec{\bm{J}}}
%\def\KV{\vec{\bm{K}}}
%\def\LV{\vec{\bm{L}}}
%\def\MV{\vec{\bm{M}}}
%\def\NV{\vec{\bm{N}}}
%\def\OV{\vec{\bm{O}}}
%\def\PV{\vec{\bm{P}}}
%\def\QV{\vec{\bm{Q}}}
%\def\RV{\vec{\bm{R}}}
%\def\SV{\vec{\bm{S}}}
%\def\TV{\vec{\bm{T}}}
%\def\UV{\vec{\bm{U}}}
%\def\VV{\vec{\bm{V}}}
%\def\WV{\vec{\bm{W}}}
%\def\XV{\vec{\bm{X}}}
%\def\YV{\vec{\bm{Y}}}
%\def\ZV{\vec{\bm{Z}}}
%
%% bold acute
%\def\aA{\acute{\bm{a}}}
%\def\bA{\acute{\bm{b}}}
%\def\cA{\acute{\bm{c}}}
%\def\dA{\acute{\bm{d}}}
%\def\eA{\acute{\bm{e}}}
%\def\fA{\acute{\bm{f}}}
%\def\gA{\acute{\bm{g}}}
%\def\hA{\acute{\bm{h}}}
%\def\iA{\acute{\bm{i}}}
%\def\iA{\acute{\bm{j}}}
%\def\kA{\acute{\bm{k}}}
%\def\lA{\acute{\bm{l}}}
%\def\mA{\acute{\bm{m}}}
%\def\nA{\acute{\bm{n}}}
%\def\oA{\acute{\bm{o}}}
%\def\pA{\acute{\bm{p}}}
%\def\qA{\acute{\bm{q}}}
%\def\rA{\acute{\bm{r}}}
%\def\sA{\acute{\bm{s}}}
%\def\tA{\acute{\bm{t}}}
%\def\uA{\acute{\bm{u}}}
%\def\vA{\acute{\bm{v}}}
%\def\wA{\acute{\bm{w}}}
%\def\xA{\acute{\bm{x}}}
%\def\yA{\acute{\bm{y}}}
%\def\zA{\acute{\bm{z}}}
%\def\AA{\acute{\bm{A}}}
%\def\BA{\acute{\bm{B}}}
%\def\CA{\acute{\bm{C}}}
%\def\DA{\acute{\bm{D}}}
%\def\EA{\acute{\bm{E}}}
%\def\FA{\acute{\bm{F}}}
%\def\GA{\acute{\bm{G}}}
%\def\HA{\acute{\bm{H}}}
%\def\IA{\acute{\bm{I}}}
%\def\JA{\acute{\bm{J}}}
%\def\KA{\acute{\bm{K}}}
%\def\LA{\acute{\bm{L}}}
%\def\MA{\acute{\bm{M}}}
%\def\NA{\acute{\bm{N}}}
%\def\OA{\acute{\bm{O}}}
%\def\PA{\acute{\bm{P}}}
%\def\QA{\acute{\bm{Q}}}
%\def\RA{\acute{\bm{R}}}
%\def\SA{\acute{\bm{S}}}
%\def\TA{\acute{\bm{T}}}
%\def\UA{\acute{\bm{U}}}
%\def\VA{\acute{\bm{V}}}
%\def\WA{\acute{\bm{W}}}
%\def\XA{\acute{\bm{X}}}
%\def\YA{\acute{\bm{Y}}}
%\def\ZA{\acute{\bm{Z}}}
%
%% bold check
%\def\aC{\check{\bm{a}}}
%\def\bC{\check{\bm{b}}}
%\def\cC{\check{\bm{c}}}
%\def\dC{\check{\bm{d}}}
%\def\eC{\check{\bm{e}}}
%\def\fC{\check{\bm{f}}}
%\def\gC{\check{\bm{g}}}
%\def\hC{\check{\bm{h}}}
%\def\iC{\check{\bm{i}}}
%\def\iC{\check{\bm{j}}}
%\def\kC{\check{\bm{k}}}
%\def\lC{\check{\bm{l}}}
%\def\mC{\check{\bm{m}}}
%\def\nC{\check{\bm{n}}}
%\def\oC{\check{\bm{o}}}
%\def\pC{\check{\bm{p}}}
%\def\qC{\check{\bm{q}}}
%\def\rC{\check{\bm{r}}}
%\def\sC{\check{\bm{s}}}
%\def\tC{\check{\bm{t}}}
%\def\uC{\check{\bm{u}}}
%\def\vC{\check{\bm{v}}}
%\def\wC{\check{\bm{w}}}
%\def\xC{\check{\bm{x}}}
%\def\yC{\check{\bm{y}}}
%\def\zC{\check{\bm{z}}}
%\def\AC{\check{\bm{A}}}
%\def\BC{\check{\bm{B}}}
%\def\CC{\check{\bm{C}}}
%\def\DC{\check{\bm{D}}}
%\def\EC{\check{\bm{E}}}
%\def\FC{\check{\bm{F}}}
%\def\GC{\check{\bm{G}}}
%\def\HC{\check{\bm{H}}}
%\def\IC{\check{\bm{I}}}
%\def\JC{\check{\bm{J}}}
%\def\KC{\check{\bm{K}}}
%\def\LC{\check{\bm{L}}}
%\def\MC{\check{\bm{M}}}
%\def\NC{\check{\bm{N}}}
%\def\OC{\check{\bm{O}}}
%\def\PC{\check{\bm{P}}}
%\def\QC{\check{\bm{Q}}}
%\def\RC{\check{\bm{R}}}
%\def\SC{\check{\bm{S}}}
%\def\TC{\check{\bm{T}}}
%\def\UC{\check{\bm{U}}}
%\def\VC{\check{\bm{V}}}
%\def\WC{\check{\bm{W}}}
%\def\XC{\check{\bm{X}}}
%\def\YC{\check{\bm{Y}}}
%\def\ZC{\check{\bm{Z}}}
%
%
%% bold dot
%\def\aD{\dot{\bm{a}}}
%\def\bD{\dot{\bm{b}}}
%\def\cD{\dot{\bm{c}}}
%\def\dD{\dot{\bm{d}}}
%\def\eD{\dot{\bm{e}}}
%\def\fD{\dot{\bm{f}}}
%\def\gD{\dot{\bm{g}}}
%\def\hD{\dot{\bm{h}}}
%\def\iD{\dot{\bm{i}}}
%\def\iD{\dot{\bm{j}}}
%\def\kD{\dot{\bm{k}}}
%\def\lD{\dot{\bm{l}}}
%\def\mD{\dot{\bm{m}}}
%\def\nD{\dot{\bm{n}}}
%\def\oD{\dot{\bm{o}}}
%\def\pD{\dot{\bm{p}}}
%\def\qD{\dot{\bm{q}}}
%\def\rD{\dot{\bm{r}}}
%\def\sD{\dot{\bm{s}}}
%\def\tD{\dot{\bm{t}}}
%\def\uD{\dot{\bm{u}}}
%\def\vD{\dot{\bm{v}}}
%\def\wD{\dot{\bm{w}}}
\def\xD{\dot{\bm{x}}}
%\def\yD{\dot{\bm{y}}}
%\def\zD{\dot{\bm{z}}}
%\def\AD{\dot{\bm{A}}}
%\def\BD{\dot{\bm{B}}}
%\def\CD{\dot{\bm{C}}}
%\def\DD{\dot{\bm{D}}}
%\def\ED{\dot{\bm{E}}}
%\def\FD{\dot{\bm{F}}}
%\def\GD{\dot{\bm{G}}}
%\def\HD{\dot{\bm{H}}}
%\def\ID{\dot{\bm{I}}}
%\def\JD{\dot{\bm{J}}}
%\def\KD{\dot{\bm{K}}}
%\def\LD{\dot{\bm{L}}}
%\def\MD{\dot{\bm{M}}}
%\def\ND{\dot{\bm{N}}}
%\def\OD{\dot{\bm{O}}}
%\def\PD{\dot{\bm{P}}}
%\def\QD{\dot{\bm{Q}}}
%\def\RD{\dot{\bm{R}}}
%\def\SD{\dot{\bm{S}}}
%\def\TD{\dot{\bm{T}}}
%\def\UD{\dot{\bm{U}}}
%\def\VD{\dot{\bm{V}}}
%\def\WD{\dot{\bm{W}}}
%\def\XD{\dot{\bm{X}}}
%\def\YD{\dot{\bm{Y}}}
%\def\ZD{\dot{\bm{Z}}}
%
%
%% bold double dot
%\def\aDD{\ddot{\bm{a}}}
%\def\bDD{\ddot{\bm{b}}}
%\def\cDD{\ddot{\bm{c}}}
%\def\dDD{\ddot{\bm{d}}}
%\def\eDD{\ddot{\bm{e}}}
%\def\fDD{\ddot{\bm{f}}}
%\def\gDD{\ddot{\bm{g}}}
%\def\hDD{\ddot{\bm{h}}}
%\def\iDD{\ddot{\bm{i}}}
%\def\iDD{\ddot{\bm{j}}}
%\def\kDD{\ddot{\bm{k}}}
%\def\lDD{\ddot{\bm{l}}}
%\def\mDD{\ddot{\bm{m}}}
%\def\nDD{\ddot{\bm{n}}}
%\def\oDD{\ddot{\bm{o}}}
%\def\pDD{\ddot{\bm{p}}}
%\def\qDD{\ddot{\bm{q}}}
%\def\rDD{\ddot{\bm{r}}}
%\def\sDD{\ddot{\bm{s}}}
%\def\tDD{\ddot{\bm{t}}}
%\def\uDD{\ddot{\bm{u}}}
%\def\vDD{\ddot{\bm{v}}}
%\def\wDD{\ddot{\bm{w}}}
%\def\xDD{\ddot{\bm{x}}}
%\def\yDD{\ddot{\bm{y}}}
%\def\zDD{\ddot{\bm{z}}}
%\def\ADD{\ddot{\bm{A}}}
%\def\BDD{\ddot{\bm{B}}}
%\def\CDD{\ddot{\bm{C}}}
%\def\DDD{\ddot{\bm{D}}}
%\def\EDD{\ddot{\bm{E}}}
%\def\FDD{\ddot{\bm{F}}}
%\def\GDD{\ddot{\bm{G}}}
%\def\HDD{\ddot{\bm{H}}}
%\def\IDD{\ddot{\bm{I}}}
%\def\JDD{\ddot{\bm{J}}}
%\def\KDD{\ddot{\bm{K}}}
%\def\LDD{\ddot{\bm{L}}}
%\def\MDD{\ddot{\bm{M}}}
%\def\NDD{\ddot{\bm{N}}}
%\def\ODD{\ddot{\bm{O}}}
%\def\PDD{\ddot{\bm{P}}}
%\def\QDD{\ddot{\bm{Q}}}
%\def\RDD{\ddot{\bm{R}}}
%\def\SDD{\ddot{\bm{S}}}
%\def\TDD{\ddot{\bm{T}}}
%\def\UDD{\ddot{\bm{U}}}
%\def\VDD{\ddot{\bm{V}}}
%\def\WDD{\ddot{\bm{W}}}
%\def\XDD{\ddot{\bm{X}}}
%\def\YDD{\ddot{\bm{Y}}}
%\def\ZDD{\ddot{\bm{Z}}}
%
%
% hat
\def\ah{\hat{{a}}}
\def\bh{\hat{{b}}}
\def\ch{\hat{{c}}}
\def\dh{\hat{{d}}}
\def\eh{\hat{{e}}}
\def\fh{\hat{{f}}}
\def\gh{\hat{{g}}}
\def\hh{\hat{{h}}}
\def\ih{\hat{{i}}}
\def\jh{\hat{{j}}}
\def\kh{\hat{{k}}}
\def\lh{\hat{{l}}}
\def\mh{\hat{{m}}}
\def\nh{\hat{{n}}}
\def\oh{\hat{{o}}}
\def\ph{\hat{{p}}}
\def\qh{\hat{{q}}}
\def\rh{\hat{{r}}}
\def\sh{\hat{{s}}}
\def\th{\hat{{t}}}
\def\uh{\hat{{u}}}
\def\vh{\hat{{v}}}
\def\wh{\hat{{w}}}
\def\xh{\hat{{x}}}
\def\yh{\hat{{y}}}
\def\zh{\hat{{z}}}
\def\Ah{\hat{{A}}}
\def\Bh{\hat{{B}}}
\def\Ch{\hat{{C}}}
\def\Dh{\hat{{D}}}
\def\Eh{\hat{{E}}}
\def\Fh{\hat{{F}}}
\def\Gh{\hat{{G}}}
\def\Hh{\hat{{H}}}
\def\Ih{\hat{{I}}}
\def\Jh{\hat{{J}}}
\def\Kh{\hat{{K}}}
\def\Lh{\hat{{L}}}
\def\Mh{\hat{{M}}}
\def\Nh{\hat{{N}}}
\def\Oh{\hat{{O}}}
\def\Ph{\hat{{P}}}
\def\Qh{\hat{{Q}}}
\def\Rh{\hat{{R}}}
\def\Sh{\hat{{S}}}
\def\Th{\hat{{T}}}
\def\Uh{\hat{{U}}}
\def\Vh{\hat{{V}}}
\def\Wh{\hat{{W}}}
\def\Xh{\hat{{X}}}
\def\Yh{\hat{{Y}}}
\def\Zh{\hat{{Z}}}
%% hat of greek letters
\def\rhoh{\hat{\rho}}
\def\pih{\hat{\pi}}
\def\tauh{\hat{\tau}}
%
%% bar
%\def\ab{\bar{{a}}}
%\def\bb{\bar{{b}}}
%\def\cb{\bar{{c}}}
\def\db{\bar{{d}}}
%\def\eb{\bar{{e}}}
%\def\fb{\bar{{f}}}
%\def\gb{\bar{{g}}}
%\def\hb{\bar{{h}}}
%\def\ib{\bar{{i}}}
%\def\ib{\bar{{j}}}
%\def\kb{\bar{{k}}}
%\def\lb{\bar{{l}}}
%\def\mb{\bar{{m}}}
%\def\nb{\bar{{n}}}
%\def\ob{\bar{{o}}}
%\def\pb{\bar{{p}}}
%\def\qb{\bar{{q}}}
%\def\rb{\bar{{r}}}
%\def\sb{\bar{{s}}}
%\def\tb{\bar{{t}}}
%\def\ub{\bar{{u}}}
%\def\vb{\bar{{v}}}
%\def\wb{\bar{{w}}}
%\def\xb{\bar{{x}}}
\def\yb{\bar{{y}}}
%\def\zb{\bar{{z}}}
%\def\Ab{\bar{{A}}}
%\def\Bb{\bar{{B}}}
%\def\Cb{\bar{{C}}}
%\def\Db{\bar{{D}}}
%\def\Eb{\bar{{E}}}
%\def\Fb{\bar{{F}}}
%\def\Gb{\bar{{G}}}
%\def\Hb{\bar{{H}}}
%\def\Ib{\bar{{I}}}
%\def\Jb{\bar{{J}}}
%\def\Kb{\bar{{K}}}
%\def\Lb{\bar{{L}}}
%\def\Mb{\bar{{M}}}
%\def\Nb{\bar{{N}}}
%\def\Ob{\bar{{O}}}
%\def\Pb{\bar{{P}}}
%\def\Qb{\bar{{Q}}}
%\def\Rb{\bar{{R}}}
%\def\Sb{\bar{{S}}}
%\def\Tb{\bar{{T}}}
%\def\Ub{\bar{{U}}}
%\def\Vb{\bar{{V}}}
%\def\Wb{\bar{{W}}}
%\def\Xb{\bar{{X}}}
%\def\Yb{\bar{{Y}}}
%\def\Zb{\bar{{Z}}}
%
%%% tilde
%%\def\at{\tilde{{a}}}
%%\def\bt{\tilde{{b}}}
%%\def\ct{\tilde{{c}}}
%%\def\dt{\tilde{{d}}}
%%\def\et{\tilde{{e}}}
%%\def\ft{\tilde{{f}}}
%%\def\gt{\tilde{{g}}}
%%\def\htilde{\tilde{{h}}}
%%\def\it{\tilde{{i}}}
%%\def\it{\tilde{{j}}}
%%\def\kt{\tilde{{k}}}
%%\def\lt{\tilde{{l}}}
%%\def\mt{\tilde{{m}}}
%%\def\nt{\tilde{{n}}}
%%\def\ot{\tilde{{o}}}
%%\def\pt{\tilde{{p}}}
%%\def\qt{\tilde{{q}}}
%%\def\rt{\tilde{{r}}}
%%\def\st{\tilde{{s}}}
%%\def\tt{\tilde{{t}}}
%%\def\ut{\tilde{{u}}}
%%\def\vt{\tilde{{v}}}
%%\def\wt{\tilde{{w}}}
%%\def\xt{\tilde{{x}}}
%%\def\yt{\tilde{{y}}}
%%\def\zt{\tilde{{z}}}
%%\def\At{\tilde{{A}}}
%%\def\Bt{\tilde{{B}}}
%%\def\Ct{\tilde{{C}}}
%%\def\Dt{\tilde{{D}}}
%%\def\Et{\tilde{{E}}}
%%\def\Ft{\tilde{{F}}}
%%\def\Gt{\tilde{{G}}}
%%\def\Ht{\tilde{{H}}}
%%\def\It{\tilde{{I}}}
%%\def\Jt{\tilde{{J}}}
%%\def\Kt{\tilde{{K}}}
%%\def\Lt{\tilde{{L}}}
%%\def\Mt{\tilde{{M}}}
%%\def\Nt{\tilde{{N}}}
%%\def\Ot{\tilde{{O}}}
%%\def\Pt{\tilde{{P}}}
%%\def\Qt{\tilde{{Q}}}
%%\def\Rt{\tilde{{R}}}
%%\def\St{\tilde{{S}}}
%%\def\Tt{\tilde{{T}}}
%%\def\Ut{\tilde{{U}}}
%%\def\Vt{\tilde{{V}}}
%%\def\Wt{\tilde{{W}}}
%%\def\Xt{\tilde{{X}}}
%%\def\Yt{\tilde{{Y}}}
%%\def\Zt{\tilde{{Z}}}
%
%% vec
%\def\av{\vec{{a}}}
%\def\bv{\vec{{b}}}
%\def\cv{\vec{{c}}}
%\def\dv{\vec{{d}}}
%\def\ev{\vec{{e}}}
%\def\fv{\vec{{f}}}
%\def\gv{\vec{{g}}}
%\def\hv{\vec{{h}}}
%\def\iv{\vec{{i}}}
%\def\iv{\vec{{j}}}
%\def\kv{\vec{{k}}}
%\def\lv{\vec{{l}}}
%\def\mv{\vec{{m}}}
%\def\nv{\vec{{n}}}
%\def\ov{\vec{{o}}}
%\def\pv{\vec{{p}}}
%\def\qv{\vec{{q}}}
%\def\rv{\vec{{r}}}
%\def\sv{\vec{{s}}}
%\def\tv{\vec{{t}}}
%\def\uv{\vec{{u}}}
%\def\vv{\vec{{v}}}
%\def\wv{\vec{{w}}}
%\def\xv{\vec{{x}}}
%\def\yv{\vec{{y}}}
%\def\zv{\vec{{z}}}
%\def\Av{\vec{{A}}}
%\def\Bv{\vec{{B}}}
%\def\Cv{\vec{{C}}}
%\def\Dv{\vec{{D}}}
%\def\Ev{\vec{{E}}}
%\def\Fv{\vec{{F}}}
%\def\Gv{\vec{{G}}}
%\def\hv{\vec{{h}}}
%\def\Iv{\vec{{I}}}
%\def\Jv{\vec{{J}}}
%\def\Kv{\vec{{K}}}
%\def\Lv{\vec{{L}}}
%\def\Mv{\vec{{M}}}
%\def\Nv{\vec{{N}}}
%\def\Ov{\vec{{O}}}
%\def\Pv{\vec{{P}}}
%\def\Qv{\vec{{Q}}}
%\def\Rv{\vec{{R}}}
%\def\Sv{\vec{{S}}}
%\def\Tv{\vec{{T}}}
%\def\Uv{\vec{{U}}}
%\def\Vv{\vec{{V}}}
%\def\Wv{\vec{{W}}}
%\def\Xv{\vec{{X}}}
%\def\Yv{\vec{{Y}}}
%\def\Zv{\vec{{Z}}}
%
%% acute
%\def\aa{\acute{{a}}}
%\def\ba{\acute{{b}}}
%\def\ca{\acute{{c}}}
%\def\da{\acute{{d}}}
%\def\ea{\acute{{e}}}
%\def\fa{\acute{{f}}}
%\def\ga{\acute{{g}}}
%\def\ha{\acute{{h}}}
%\def\ia{\acute{{i}}}
%\def\ia{\acute{{j}}}
%\def\ka{\acute{{k}}}
%\def\la{\acute{{l}}}
%\def\ma{\acute{{m}}}
%\def\na{\acute{{n}}}
%\def\oa{\acute{{o}}}
%\def\pa{\acute{{p}}}
%\def\qa{\acute{{q}}}
%\def\ra{\acute{{r}}}
%\def\sa{\acute{{s}}}
%\def\ta{\acute{{t}}}
%\def\ua{\acute{{u}}}
%\def\va{\acute{{v}}}
%\def\wa{\acute{{w}}}
%\def\xa{\acute{{x}}}
%\def\ya{\acute{{y}}}
%\def\za{\acute{{z}}}
%\def\Aa{\acute{{A}}}
%\def\Ba{\acute{{B}}}
%\def\Ca{\acute{{C}}}
%\def\Da{\acute{{D}}}
%\def\Ea{\acute{{E}}}
%\def\Fa{\acute{{F}}}
%\def\Ga{\acute{{G}}}
%\def\Ha{\acute{{H}}}
%\def\Ia{\acute{{I}}}
%\def\Ja{\acute{{J}}}
%\def\Ka{\acute{{K}}}
%\def\La{\acute{{L}}}
%\def\Ma{\acute{{M}}}
%\def\Na{\acute{{N}}}
%\def\Oa{\acute{{O}}}
%\def\Pa{\acute{{P}}}
%\def\Qa{\acute{{Q}}}
%\def\Ra{\acute{{R}}}
%\def\Sa{\acute{{S}}}
%\def\Ta{\acute{{T}}}
%\def\Ua{\acute{{U}}}
%\def\Va{\acute{{V}}}
%\def\Wa{\acute{{W}}}
%\def\Xa{\acute{{X}}}
%\def\Ya{\acute{{Y}}}
%\def\Za{\acute{{Z}}}
%
%% check
%\def\ac{\check{{a}}}
%\def\bc{\check{{b}}}
%\def\cc{\check{{c}}}
%\def\dc{\check{{d}}}
%\def\ec{\check{{e}}}
%\def\fc{\check{{f}}}
%\def\gc{\check{{g}}}
%\def\hc{\check{{h}}}
%\def\ic{\check{{i}}}
%\def\ic{\check{{j}}}
%\def\kc{\check{{k}}}
%\def\lc{\check{{l}}}
%\def\mc{\check{{m}}}
%\def\nc{\check{{n}}}
%\def\oc{\check{{o}}}
%\def\pc{\check{{p}}}
%\def\qc{\check{{q}}}
%\def\rc{\check{{r}}}
%\def\sc{\check{{s}}}
%\def\tc{\check{{t}}}
%\def\uc{\check{{u}}}
%\def\vc{\check{{v}}}
%\def\wc{\check{{w}}}
%\def\xc{\check{{x}}}
%\def\yc{\check{{y}}}
%\def\zc{\check{{z}}}
%\def\Ac{\check{{A}}}
%\def\Bc{\check{{B}}}
%\def\Cc{\check{{C}}}
%\def\Dc{\check{{D}}}
%\def\Ec{\check{{E}}}
%\def\Fc{\check{{F}}}
%\def\Gc{\check{{G}}}
%\def\Hc{\check{{H}}}
%\def\Ic{\check{{I}}}
%\def\Jc{\check{{J}}}
%\def\Kc{\check{{K}}}
%\def\Lc{\check{{L}}}
%\def\Mc{\check{{M}}}
%\def\Nc{\check{{N}}}
%\def\Oc{\check{{O}}}
%\def\Pc{\check{{P}}}
%\def\Qc{\check{{Q}}}
%\def\Rc{\check{{R}}}
%\def\Sc{\check{{S}}}
%\def\Tc{\check{{T}}}
%\def\Uc{\check{{U}}}
%\def\Vc{\check{{V}}}
%\def\Wc{\check{{W}}}
%\def\Xc{\check{{X}}}
%\def\Yc{\check{{Y}}}
%\def\Zc{\check{{Z}}}
%
%
%% dot
\def\ad{\dot{{a}}}
\def\bd{\dot{{b}}}
\def\cd{\dot{{c}}}
\def\dd{\dot{{d}}}
\def\ed{\dot{{e}}}
\def\fd{\dot{{f}}}
\def\gd{\dot{{g}}}
\def\hd{\dot{{h}}}
\def\id{\dot{{i}}}
\def\id{\dot{{j}}}
\def\kd{\dot{{k}}}
\def\ld{\dot{{l}}}
\def\md{\dot{{m}}}
\def\nd{\dot{{n}}}
\def\od{\dot{{o}}}
\def\pd{\dot{{p}}}
\def\qd{\dot{{q}}}
\def\rd{\dot{{r}}}
\def\sd{\dot{{s}}}
\def\td{\dot{{t}}}
\def\ud{\dot{{u}}}
\def\vd{\dot{{v}}}
\def\wdot{\dot{{w}}}
\def\xd{\dot{{x}}}
\def\yd{\dot{{y}}}
\def\zd{\dot{{z}}}
\def\Ad{\dot{{A}}}
\def\Bd{\dot{{B}}}
\def\Cd{\dot{{C}}}
\def\Dd{\dot{{D}}}
\def\Ed{\dot{{E}}}
\def\Fd{\dot{{F}}}
\def\Gd{\dot{{G}}}
\def\Hd{\dot{{H}}}
\def\Id{\dot{{I}}}
\def\Jd{\dot{{J}}}
\def\Kd{\dot{{K}}}
\def\Ld{\dot{{L}}}
\def\Md{\dot{{M}}}
\def\Nd{\dot{{N}}}
\def\Od{\dot{{O}}}
\def\Pd{\dot{{P}}}
\def\Qd{\dot{{Q}}}
\def\Rd{\dot{{R}}}
\def\Sd{\dot{{S}}}
\def\Td{\dot{{T}}}
\def\Ud{\dot{{U}}}
\def\Vd{\dot{{V}}}
\def\Wd{\dot{{W}}}
\def\Xd{\dot{{X}}}
\def\Yd{\dot{{Y}}}
\def\Zd{\dot{{Z}}}
%
%
%% double dot
%\def\add{\ddot{{a}}}
%\def\bdd{\ddot{{b}}}
%\def\cdd{\ddot{{c}}}
%\def\ddd{\ddot{{d}}}
%\def\edd{\ddot{{e}}}
%\def\fdd{\ddot{{f}}}
%\def\gdd{\ddot{{g}}}
%\def\hdd{\ddot{{h}}}
%\def\idd{\ddot{{i}}}
%\def\idd{\ddot{{j}}}
%\def\kdd{\ddot{{k}}}
%\def\ldd{\ddot{{l}}}
%\def\mdd{\ddot{{m}}}
%\def\ndd{\ddot{{n}}}
%\def\odd{\ddot{{o}}}
%\def\pdd{\ddot{{p}}}
%\def\qdd{\ddot{{q}}}
%\def\rdd{\ddot{{r}}}
%\def\sdd{\ddot{{s}}}
%\def\tdd{\ddot{{t}}}
%\def\udd{\ddot{{u}}}
%\def\vdd{\ddot{{v}}}
%\def\wdd{\ddot{{w}}}
%\def\xdd{\ddot{{x}}}
%\def\ydd{\ddot{{y}}}
%\def\zdd{\ddot{{z}}}
%\def\Add{\ddot{{A}}}
%\def\Bdd{\ddot{{B}}}
%\def\Cdd{\ddot{{C}}}
%\def\Ddd{\ddot{{D}}}
%\def\Edd{\ddot{{E}}}
%\def\Fdd{\ddot{{F}}}
%\def\Gdd{\ddot{{G}}}
%\def\Hdd{\ddot{{H}}}
%\def\Idd{\ddot{{I}}}
%\def\Jdd{\ddot{{J}}}
%\def\Kdd{\ddot{{K}}}
%\def\Ldd{\ddot{{L}}}
%\def\Mdd{\ddot{{M}}}
%\def\Ndd{\ddot{{N}}}
%\def\Odd{\ddot{{O}}}
%\def\Pdd{\ddot{{P}}}
%\def\Qdd{\ddot{{Q}}}
%\def\Rdd{\ddot{{R}}}
%\def\Sdd{\ddot{{S}}}
%\def\Tdd{\ddot{{T}}}
%\def\Udd{\ddot{{U}}}
%\def\Vdd{\ddot{{V}}}
%\def\Wdd{\ddot{{W}}}
%\def\Xdd{\ddot{{X}}}
%\def\Ydd{\ddot{{Y}}}
%\def\Zdd{\ddot{{Z}}}
%
%
%% script 
\def\as{\mathcal{{a}}}
\def\bs{\mathcal{{b}}}
\def\cs{\mathcal{{c}}}
\def\ds{\mathcal{{d}}}
\def\es{\mathcal{{e}}}
\def\fs{\mathcal{{f}}}
\def\gs{\mathcal{{g}}}
\def\hs{\mathcal{{h}}}
\def\is{\mathcal{{i}}}
\def\is{\mathcal{{j}}}
\def\ks{\mathcal{{k}}}
\def\ls{\mathcal{{l}}}
\def\ms{\mathcal{{m}}}
\def\ns{\mathcal{{n}}}
\def\os{\mathcal{{o}}}
\def\ps{\mathcal{{p}}}
\def\qs{\mathcal{{q}}}
\def\rs{\mathcal{{r}}}
\def\ss{\mathcal{{s}}}
\def\ts{\mathcal{{t}}}
\def\us{\mathcal{{u}}}
\def\vs{\mathcal{{v}}}
\def\ws{\mathcal{{w}}}
\def\xs{\mathcal{{x}}}
\def\ys{\mathcal{{y}}}
\def\zs{\mathcal{{z}}}
\def\As{\mathcal{{A}}}
\def\Bs{\mathcal{{B}}}
\def\Cs{\mathcal{{C}}}
\def\Ds{\mathcal{{D}}}
\def\Dsh{\hat{\mathcal{{D}}}}
\def\Es{\mathcal{{E}}}
\def\Fs{\mathcal{{F}}}
\def\Gs{\mathcal{{G}}}
\def\Gsh{\hat{\mathcal{{G}}}}
\def\Hs{\mathcal{{H}}}
\def\Hsh{\hat{\mathcal{{H}}}}
\def\Is{\mathcal{{I}}}
\def\Js{\mathcal{{J}}}
\def\Ks{\mathcal{{K}}}
\def\Ksh{\hat{\mathcal{{K}}}}
\def\Ksb{\bar{\mathcal{{K}}}}
\def\Ls{\mathcal{{L}}}
\def\Ms{\mathcal{{M}}}
\def\Ns{\mathcal{{N}}}
\def\Os{\mathcal{{O}}}
\def\Ps{\mathcal{{P}}}
\def\Qs{\mathcal{{Q}}}
\def\Rs{\mathcal{{R}}}
\def\Ss{\mathcal{{S}}}
\def\Ts{\mathcal{{T}}}
\def\Us{\mathcal{{U}}}
\def\Vs{\mathcal{{V}}}
\def\Ws{\mathcal{{W}}}
\def\Xs{\mathcal{{X}}}
\def\Ys{\mathcal{{Y}}}
\def\Zs{\mathcal{{Z}}}
%

%% script hat
\def\Fsh{\hat{\Fs}}

%
%% bold greeks
\def\alphaB{{\bm{\alpha}}}
\def\betaB{{\bm{\beta}}}
\def\gammaB{{\bm{\gamma}}}
\def\deltaB{{\bm{\delta}}}
\def\epsilonB{{\bm{\epsilon}}}
\def\zetaB{{\bm{\zeta}}}
\def\etaB{{\bm{\eta}}}
\def\thetaB{{\bm{\theta}}}
\def\iotaB{{\bm{\iota}}}
\def\kappaB{{\bm{\kappa}}}
\def\lambdaB{{\bm{\lambda}}}
\def\muB{{\bm{\mu}}}
\def\nuB{{\bm{\nu}}}
\def\piB{{\bm{\pi}}}
\def\rhoB{{\bm{\rho}}}
\def\sigmaB{{\bm{\sigma}}}
\def\tauB{{\bm{\tau}}}
\def\upsilonB{{\bm{\upsilon}}}
\def\phiB{{\bm{\phi}}}
\def\chiB{{\bm{\chi}}}
\def\psiB{{\bm{\psi}}}
\def\omegaB{{\bm{\omega}}}
\def\GammaB{{\bm{\Gamma}}}
\def\DeltaB{{\bm{\Delta}}}
\def\ThetaB{{\bm{\Theta}}}
\def\LambdaB{{\bm{\Lambda}}}
\def\PiB{{\bm{\Pi}}}
\def\SigmaB{{\bm{\Sigma}}}
\def\UpsilonB{{\bm{\Upsilon}}}
\def\PhiB{{\bm{\Phi}}}
\def\PsiB{{\bm{\Psi}}}
\def\OmegaB{{\bm{\Omega}}}
%
%
%% bold hat greeks
%\def\alphaBH{\hat{\bm{\alpha}}}
%\def\betaBH{\hat{\bm{\beta}}}
\def\gammaBH{\hat{\bm{\gamma}}}
%\def\deltaBH{\hat{\bm{\delta}}}
%\def\epsilonBH{\hat{\bm{\epsilon}}}
%\def\zetaBH{\hat{\bm{\zeta}}}
%\def\etaBH{\hat{\bm{\eta}}}
\def\thetaBH{\hat{\bm{\theta}}}
%\def\iotaBH{\hat{\bm{\iota}}}
%\def\kappaBH{\hat{\bm{\kappa}}}
%\def\lambdaBH{\hat{\bm{\lambda}}}
%\def\muBH{\hat{\bm{\mu}}}
%\def\nuBH{\hat{\bm{\nu}}}
%\def\piBH{\hat{\bm{\pi}}}
%\def\rhoBH{\hat{\bm{\rho}}}
%\def\sigmaBH{\hat{\bm{\sigma}}}
%\def\tauBH{\hat{\bm{\tau}}}
%\def\upsilonBH{\hat{\bm{\upsilon}}}
%\def\phiBH{\hat{\bm{\phi}}}
%\def\chiBH{\hat{\bm{\chi}}}
%\def\psiBH{\hat{\bm{\psi}}}
%\def\omegaBH{\hat{\bm{\omega}}}
%\def\GammaBH{\hat{\bm{\Gamma}}}
%\def\DeltaBH{\hat{\bm{\Delta}}}
%\def\ThetaBH{\hat{\bm{\Theta}}}
%\def\LambdaBH{\hat{\bm{\Lambda}}}
%\def\PiBH{\hat{\bm{\Pi}}}
%\def\SigmaBH{\hat{\bm{\Sigma}}}
%\def\UpsilonBH{\hat{\bm{\Upsilon}}}
%\def\PhiBH{\hat{\bm{\Phi}}}
%\def\PsiBH{\hat{\bm{\Psi}}}
%\def\OmegaBH{\hat{\bm{\Omega}}}
%
%
%% bold bar greeks
%\def\alphaBB{\bar{\bm{\alpha}}}
%\def\betaBB{\bar{\bm{\beta}}}
%\def\gammaBB{\bar{\bm{\gamma}}}
%\def\deltaBB{\bar{\bm{\delta}}}
%\def\epsilonBB{\bar{\bm{\epsilon}}}
%\def\zetaBB{\bar{\bm{\zeta}}}
%\def\etaBB{\bar{\bm{\eta}}}
\def\thetaBB{\bar{\bm{\theta}}}
%\def\iotaBB{\bar{\bm{\iota}}}
%\def\kappaBB{\bar{\bm{\kappa}}}
%\def\lambdaBB{\bar{\bm{\lambda}}}
%\def\muBB{\bar{\bm{\mu}}}
%\def\nuBB{\bar{\bm{\nu}}}
%\def\piBB{\bar{\bm{\pi}}}
%\def\rhoBB{\bar{\bm{\rho}}}
%\def\sigmaBB{\bar{\bm{\sigma}}}
%\def\tauBB{\bar{\bm{\tau}}}
%\def\upsilonBB{\bar{\bm{\upsilon}}}
%\def\phiBB{\bar{\bm{\phi}}}
%\def\chiBB{\bar{\bm{\chi}}}
%\def\psiBB{\bar{\bm{\psi}}}
%\def\omegaBB{\bar{\bm{\omega}}}
%\def\GammaBB{\bar{\bm{\Gamma}}}
%\def\DeltaBB{\bar{\bm{\Delta}}}
%\def\ThetaBB{\bar{\bm{\Theta}}}
%\def\LambdaBB{\bar{\bm{\Lambda}}}
%\def\PiBB{\bar{\bm{\Pi}}}
%\def\SigmaBB{\bar{\bm{\Sigma}}}
%\def\UpsilonBB{\bar{\bm{\Upsilon}}}
%\def\PhiBB{\bar{\bm{\Phi}}}
%\def\PsiBB{\bar{\bm{\Psi}}}
%\def\OmegaBB{\bar{\bm{\Omega}}}
%
%% bold tilde greeks
%\def\alphaBT{\tilde{\bm{\alpha}}}
%\def\betaBT{\tilde{\bm{\beta}}}
%\def\gammaBT{\tilde{\bm{\gamma}}}
%\def\deltaBT{\tilde{\bm{\delta}}}
%\def\epsilonBT{\tilde{\bm{\epsilon}}}
%\def\zetaBT{\tilde{\bm{\zeta}}}
%\def\etaBT{\tilde{\bm{\eta}}}
%\def\thetaBT{\tilde{\bm{\theta}}}
%\def\iotaBT{\tilde{\bm{\iota}}}
%\def\kappaBT{\tilde{\bm{\kappa}}}
%\def\lambdaBT{\tilde{\bm{\lambda}}}
%\def\muBT{\tilde{\bm{\mu}}}
%\def\nuBT{\tilde{\bm{\nu}}}
%\def\piBT{\tilde{\bm{\pi}}}
%\def\rhoBT{\tilde{\bm{\rho}}}
%\def\sigmaBT{\tilde{\bm{\sigma}}}
%\def\tauBT{\tilde{\bm{\tau}}}
%\def\upsilonBT{\tilde{\bm{\upsilon}}}
%\def\phiBT{\tilde{\bm{\phi}}}
%\def\chiBT{\tilde{\bm{\chi}}}
%\def\psiBT{\tilde{\bm{\psi}}}
%\def\omegaBT{\tilde{\bm{\omega}}}
%\def\GammaBT{\tilde{\bm{\Gamma}}}
%\def\DeltaBT{\tilde{\bm{\Delta}}}
%\def\ThetaBT{\tilde{\bm{\Theta}}}
%\def\LambdaBT{\tilde{\bm{\Lambda}}}
%\def\PiBT{\tilde{\bm{\Pi}}}
%\def\SigmaBT{\tilde{\bm{\Sigma}}}
%\def\UpsilonBT{\tilde{\bm{\Upsilon}}}
%\def\PhiBT{\tilde{\bm{\Phi}}}
%\def\PsiBT{\tilde{\bm{\Psi}}}
%\def\OmegaBT{\tilde{\bm{\Omega}}}
%
%
%% bold vec greeks
%\def\alphaBV{\vec{\bm{\alpha}}}
%\def\betaBV{\vec{\bm{\beta}}}
%\def\gammaBV{\vec{\bm{\gamma}}}
%\def\deltaBV{\vec{\bm{\delta}}}
%\def\epsilonBV{\vec{\bm{\epsilon}}}
%\def\zetaBV{\vec{\bm{\zeta}}}
%\def\etaBV{\vec{\bm{\eta}}}
%\def\thetaBV{\vec{\bm{\theta}}}
%\def\iotaBV{\vec{\bm{\iota}}}
%\def\kappaBV{\vec{\bm{\kappa}}}
%\def\lambdaBV{\vec{\bm{\lambda}}}
%\def\muBV{\vec{\bm{\mu}}}
%\def\nuBV{\vec{\bm{\nu}}}
%\def\piBV{\vec{\bm{\pi}}}
%\def\rhoBV{\vec{\bm{\rho}}}
%\def\sigmaBV{\vec{\bm{\sigma}}}
%\def\tauBV{\vec{\bm{\tau}}}
%\def\upsilonBV{\vec{\bm{\upsilon}}}
%\def\phiBV{\vec{\bm{\phi}}}
%\def\chiBV{\vec{\bm{\chi}}}
%\def\psiBV{\vec{\bm{\psi}}}
%\def\omegaBV{\vec{\bm{\omega}}}
%\def\GammaBV{\vec{\bm{\Gamma}}}
%\def\DeltaBV{\vec{\bm{\Delta}}}
%\def\ThetaBV{\vec{\bm{\Theta}}}
%\def\LambdaBV{\vec{\bm{\Lambda}}}
%\def\PiBV{\vec{\bm{\Pi}}}
%\def\SigmaBV{\vec{\bm{\Sigma}}}
%\def\UpsilonBV{\vec{\bm{\Upsilon}}}
%\def\PhiBV{\vec{\bm{\Phi}}}
%\def\PsiBV{\vec{\bm{\Psi}}}
%\def\OmegaBV{\vec{\bm{\Omega}}}
%
%% bold acute greeks
%\def\alphaBA{\acute{\bm{\alpha}}}
%\def\betaBA{\acute{\bm{\beta}}}
%\def\gammaBA{\acute{\bm{\gamma}}}
%\def\deltaBA{\acute{\bm{\delta}}}
%\def\epsilonBA{\acute{\bm{\epsilon}}}
%\def\zetaBA{\acute{\bm{\zeta}}}
%\def\etaBA{\acute{\bm{\eta}}}
%\def\thetaBA{\acute{\bm{\theta}}}
%\def\iotaBA{\acute{\bm{\iota}}}
%\def\kappaBA{\acute{\bm{\kappa}}}
%\def\lambdaBA{\acute{\bm{\lambda}}}
%\def\muBA{\acute{\bm{\mu}}}
%\def\nuBA{\acute{\bm{\nu}}}
%\def\piBA{\acute{\bm{\pi}}}
%\def\rhoBA{\acute{\bm{\rho}}}
%\def\sigmaBA{\acute{\bm{\sigma}}}
%\def\tauBA{\acute{\bm{\tau}}}
%\def\upsilonBA{\acute{\bm{\upsilon}}}
%\def\phiBA{\acute{\bm{\phi}}}
%\def\chiBA{\acute{\bm{\chi}}}
%\def\psiBA{\acute{\bm{\psi}}}
%\def\omegaBA{\acute{\bm{\omega}}}
%\def\GammaBA{\acute{\bm{\Gamma}}}
%\def\DeltaBA{\acute{\bm{\Delta}}}
%\def\ThetaBA{\acute{\bm{\Theta}}}
%\def\LambdaBA{\acute{\bm{\Lambda}}}
%\def\PiBA{\acute{\bm{\Pi}}}
%\def\SigmaBA{\acute{\bm{\Sigma}}}
%\def\UpsilonBA{\acute{\bm{\Upsilon}}}
%\def\PhiBA{\acute{\bm{\Phi}}}
%\def\PsiBA{\acute{\bm{\Psi}}}
%\def\OmegaBA{\acute{\bm{\Omega}}}
%
%
%% bold check greeks
%\def\alphaBC{\check{\bm{\alpha}}}
%\def\betaBC{\check{\bm{\beta}}}
%\def\gammaBC{\check{\bm{\gamma}}}
%\def\deltaBC{\check{\bm{\delta}}}
%\def\epsilonBC{\check{\bm{\epsilon}}}
%\def\zetaBC{\check{\bm{\zeta}}}
%\def\etaBC{\check{\bm{\eta}}}
%\def\thetaBC{\check{\bm{\theta}}}
%\def\iotaBC{\check{\bm{\iota}}}
%\def\kappaBC{\check{\bm{\kappa}}}
%\def\lambdaBC{\check{\bm{\lambda}}}
%\def\muBC{\check{\bm{\mu}}}
%\def\nuBC{\check{\bm{\nu}}}
%\def\piBC{\check{\bm{\pi}}}
%\def\rhoBC{\check{\bm{\rho}}}
%\def\sigmaBC{\check{\bm{\sigma}}}
%\def\tauBC{\check{\bm{\tau}}}
%\def\upsilonBC{\check{\bm{\upsilon}}}
%\def\phiBC{\check{\bm{\phi}}}
%\def\chiBC{\check{\bm{\chi}}}
%\def\psiBC{\check{\bm{\psi}}}
%\def\omegaBC{\check{\bm{\omega}}}
%\def\GammaBC{\check{\bm{\Gamma}}}
%\def\DeltaBC{\check{\bm{\Delta}}}
%\def\ThetaBC{\check{\bm{\Theta}}}
%\def\LambdaBC{\check{\bm{\Lambda}}}
%\def\PiBC{\check{\bm{\Pi}}}
%\def\SigmaBC{\check{\bm{\Sigma}}}
%\def\UpsilonBC{\check{\bm{\Upsilon}}}
%\def\PhiBC{\check{\bm{\Phi}}}
%\def\PsiBC{\check{\bm{\Psi}}}
%\def\OmegaBC{\check{\bm{\Omega}}}
%
%
%% bold dot greeks
%\def\alphaBD{\dot{\bm{\alpha}}}
%\def\betaBD{\dot{\bm{\beta}}}
%\def\gammaBD{\dot{\bm{\gamma}}}
%\def\deltaBD{\dot{\bm{\delta}}}
%\def\epsilonBD{\dot{\bm{\epsilon}}}
%\def\zetaBD{\dot{\bm{\zeta}}}
%\def\etaBD{\dot{\bm{\eta}}}
%\def\thetaBD{\dot{\bm{\theta}}}
%\def\iotaBD{\dot{\bm{\iota}}}
%\def\kappaBD{\dot{\bm{\kappa}}}
%\def\lambdaBD{\dot{\bm{\lambda}}}
%\def\muBD{\dot{\bm{\mu}}}
%\def\nuBD{\dot{\bm{\nu}}}
%\def\piBD{\dot{\bm{\pi}}}
%\def\rhoBD{\dot{\bm{\rho}}}
%\def\sigmaBD{\dot{\bm{\sigma}}}
%\def\tauBD{\dot{\bm{\tau}}}
%\def\upsilonBD{\dot{\bm{\upsilon}}}
%\def\phiBD{\dot{\bm{\phi}}}
%\def\chiBD{\dot{\bm{\chi}}}
%\def\psiBD{\dot{\bm{\psi}}}
%\def\omegaBD{\dot{\bm{\omega}}}
%\def\GammaBD{\dot{\bm{\Gamma}}}
%\def\DeltaBD{\dot{\bm{\Delta}}}
%\def\ThetaBD{\dot{\bm{\Theta}}}
%\def\LambdaBD{\dot{\bm{\Lambda}}}
%\def\PiBD{\dot{\bm{\Pi}}}
%\def\SigmaBD{\dot{\bm{\Sigma}}}
%\def\UpsilonBD{\dot{\bm{\Upsilon}}}
%\def\PhiBD{\dot{\bm{\Phi}}}
%\def\PsiBD{\dot{\bm{\Psi}}}
%\def\OmegaBD{\dot{\bm{\Omega}}}
%
%
%% bold double dot greeks
%\def\alphaBDD{\ddot{\bm{\alpha}}}
%\def\betaBDD{\ddot{\bm{\beta}}}
%\def\gammaBDD{\ddot{\bm{\gamma}}}
%\def\deltaBDD{\ddot{\bm{\delta}}}
%\def\epsilonBDD{\ddot{\bm{\epsilon}}}
%\def\zetaBDD{\ddot{\bm{\zeta}}}
%\def\etaBDD{\ddot{\bm{\eta}}}
%\def\thetaBDD{\ddot{\bm{\theta}}}
%\def\iotaBDD{\ddot{\bm{\iota}}}
%\def\kappaBDD{\ddot{\bm{\kappa}}}
%\def\lambdaBDD{\ddot{\bm{\lambda}}}
%\def\muBDD{\ddot{\bm{\mu}}}
%\def\nuBDD{\ddot{\bm{\nu}}}
%\def\piBDD{\ddot{\bm{\pi}}}
%\def\rhoBDD{\ddot{\bm{\rho}}}
%\def\sigmaBDD{\ddot{\bm{\sigma}}}
%\def\tauBDD{\ddot{\bm{\tau}}}
%\def\upsilonBDD{\ddot{\bm{\upsilon}}}
%\def\phiBDD{\ddot{\bm{\phi}}}
%\def\chiBDD{\ddot{\bm{\chi}}}
%\def\psiBDD{\ddot{\bm{\psi}}}
%\def\omegaBDD{\ddot{\bm{\omega}}}
%\def\GammaBDD{\ddot{\bm{\Gamma}}}
%\def\DeltaBDD{\ddot{\bm{\Delta}}}
%\def\ThetaBDD{\ddot{\bm{\Theta}}}
%\def\LambdaBDD{\ddot{\bm{\Lambda}}}
%\def\PiBDD{\ddot{\bm{\Pi}}}
%\def\SigmaBDD{\ddot{\bm{\Sigma}}}
%\def\UpsilonBDD{\ddot{\bm{\Upsilon}}}
%\def\PhiBDD{\ddot{\bm{\Phi}}}
%\def\PsiBDD{\ddot{\bm{\Psi}}}
%\def\OmegaBDD{\ddot{\bm{\Omega}}}
%
%
%
%%  hat greeks
\def\alphah{\hat{{\alpha}}}
\def\betah{\hat{{\beta}}}
\def\gammah{\hat{{\gamma}}}
\def\deltah{\hat{{\delta}}}
\def\epsilonh{\hat{{\epsilon}}}
\def\zetah{\hat{{\zeta}}}
\def\etah{\hat{{\eta}}}
\def\thetah{\hat{{\theta}}}
\def\iotah{\hat{{\iota}}}
\def\kappah{\hat{{\kappa}}}
\def\lambdah{\hat{{\lambda}}}
\def\muh{\hat{{\mu}}}
\def\nuh{\hat{{\nu}}}
\def\pih{\hat{{\pi}}}
\def\rhoh{\hat{{\rho}}}
\def\sigmah{\hat{{\sigma}}}
\def\tauh{\hat{{\tau}}}
\def\upsilonh{\hat{{\upsilon}}}
\def\phih{\hat{{\phi}}}
\def\chih{\hat{{\chi}}}
\def\psih{\hat{{\psi}}}
\def\omegah{\hat{{\omega}}}
\def\Gammah{\hat{{\Gamma}}}
\def\Deltah{\hat{{\Delta}}}
\def\Thetah{\hat{{\Theta}}}
\def\Lambdah{\hat{{\Lambda}}}
\def\Pih{\hat{{\Pi}}}
\def\Sigmah{\hat{{\Sigma}}}
\def\Upsilonh{\hat{{\Upsilon}}}
\def\Phih{\hat{{\Phi}}}
\def\Psih{\hat{{\Psi}}}
\def\Omegah{\hat{{\Omega}}}
%
%
%%  bar greeks
%\def\alphab{\bar{{\alpha}}}
%\def\betab{\bar{{\beta}}}
%\def\gammab{\bar{{\gamma}}}
%\def\deltab{\bar{{\delta}}}
%\def\epsilonb{\bar{{\epsilon}}}
%\def\zetab{\bar{{\zeta}}}
%\def\etab{\bar{{\eta}}}
%\def\thetab{\bar{{\theta}}}
%\def\iotab{\bar{{\iota}}}
%\def\kappab{\bar{{\kappa}}}
%\def\lambdab{\bar{{\lambda}}}
%\def\mub{\bar{{\mu}}}
%\def\nub{\bar{{\nu}}}
%\def\pib{\bar{{\pi}}}
%\def\rhob{\bar{{\rho}}}
%\def\sigmab{\bar{{\sigma}}}
%\def\taub{\bar{{\tau}}}
%\def\upsilonb{\bar{{\upsilon}}}
%\def\phib{\bar{{\phi}}}
%\def\chib{\bar{{\chi}}}
%\def\psib{\bar{{\psi}}}
%\def\omegab{\bar{{\omega}}}
%\def\Gammab{\bar{{\Gamma}}}
%\def\Deltab{\bar{{\Delta}}}
%\def\Thetab{\bar{{\Theta}}}
%\def\Lambdab{\bar{{\Lambda}}}
%\def\Pib{\bar{{\Pi}}}
%\def\Sigmab{\bar{{\Sigma}}}
%\def\Upsilonb{\bar{{\Upsilon}}}
%\def\Phib{\bar{{\Phi}}}
%\def\Psib{\bar{{\Psi}}}
%\def\Omegab{\bar{{\Omega}}}
%
%%  tilde greeks
%\def\alphat{\tilde{{\alpha}}}
%\def\betat{\tilde{{\beta}}}
%\def\gammat{\tilde{{\gamma}}}
%\def\deltat{\tilde{{\delta}}}
%\def\epsilont{\tilde{{\epsilon}}}
%\def\zetat{\tilde{{\zeta}}}
%\def\etat{\tilde{{\eta}}}
%\def\thetat{\tilde{{\theta}}}
%\def\iotat{\tilde{{\iota}}}
%\def\kappat{\tilde{{\kappa}}}
%\def\lambdat{\tilde{{\lambda}}}
%\def\mut{\tilde{{\mu}}}
%\def\nut{\tilde{{\nu}}}
%\def\pit{\tilde{{\pi}}}
%\def\rhot{\tilde{{\rho}}}
%\def\sigmat{\tilde{{\sigma}}}
%\def\taut{\tilde{{\tau}}}
%\def\upsilont{\tilde{{\upsilon}}}
%\def\phit{\tilde{{\phi}}}
%\def\chit{\tilde{{\chi}}}
%\def\psit{\tilde{{\psi}}}
%\def\omegat{\tilde{{\omega}}}
%\def\Gammat{\tilde{{\Gamma}}}
%\def\Deltat{\tilde{{\Delta}}}
%\def\Thetat{\tilde{{\Theta}}}
%\def\Lambdat{\tilde{{\Lambda}}}
%\def\Pit{\tilde{{\Pi}}}
%\def\Sigmat{\tilde{{\Sigma}}}
%\def\Upsilont{\tilde{{\Upsilon}}}
%\def\Phit{\tilde{{\Phi}}}
%\def\Psit{\tilde{{\Psi}}}
%\def\Omegat{\tilde{{\Omega}}}
%
%
%%  vec greeks
%\def\alphav{\vec{{\alpha}}}
%\def\betav{\vec{{\beta}}}
%\def\gammav{\vec{{\gamma}}}
%\def\deltav{\vec{{\delta}}}
%\def\epsilonv{\vec{{\epsilon}}}
%\def\zetav{\vec{{\zeta}}}
%\def\etav{\vec{{\eta}}}
%\def\thetav{\vec{{\theta}}}
%\def\iotav{\vec{{\iota}}}
%\def\kappav{\vec{{\kappa}}}
%\def\lambdav{\vec{{\lambda}}}
%\def\muv{\vec{{\mu}}}
%\def\nuv{\vec{{\nu}}}
%\def\piv{\vec{{\pi}}}
%\def\rhov{\vec{{\rho}}}
%\def\sigmav{\vec{{\sigma}}}
%\def\tauv{\vec{{\tau}}}
%\def\upsilonv{\vec{{\upsilon}}}
%\def\phiv{\vec{{\phi}}}
%\def\chiv{\vec{{\chi}}}
%\def\psiv{\vec{{\psi}}}
%\def\omegav{\vec{{\omega}}}
%\def\Gammav{\vec{{\Gamma}}}
%\def\Deltav{\vec{{\Delta}}}
%\def\Thetav{\vec{{\Theta}}}
%\def\Lambdav{\vec{{\Lambda}}}
%\def\Piv{\vec{{\Pi}}}
%\def\Sigmav{\vec{{\Sigma}}}
%\def\Upsilonv{\vec{{\Upsilon}}}
%\def\Phiv{\vec{{\Phi}}}
%\def\Psiv{\vec{{\Psi}}}
%\def\Omegav{\vec{{\Omega}}}
%
%%  acute greeks
%\def\alphaa{\acute{{\alpha}}}
%\def\betaa{\acute{{\beta}}}
%\def\gammaa{\acute{{\gamma}}}
%\def\deltaa{\acute{{\delta}}}
%\def\epsilona{\acute{{\epsilon}}}
%\def\zetaa{\acute{{\zeta}}}
%\def\etaa{\acute{{\eta}}}
%\def\thetaa{\acute{{\theta}}}
%\def\iotaa{\acute{{\iota}}}
%\def\kappaa{\acute{{\kappa}}}
%\def\lambdaa{\acute{{\lambda}}}
%\def\mua{\acute{{\mu}}}
%\def\nua{\acute{{\nu}}}
%\def\pia{\acute{{\pi}}}
%\def\rhoa{\acute{{\rho}}}
%\def\sigmaa{\acute{{\sigma}}}
%\def\taua{\acute{{\tau}}}
%\def\upsilona{\acute{{\upsilon}}}
%\def\phia{\acute{{\phi}}}
%\def\chia{\acute{{\chi}}}
%\def\psia{\acute{{\psi}}}
%\def\omegaa{\acute{{\omega}}}
%\def\Gammaa{\acute{{\Gamma}}}
%\def\Deltaa{\acute{{\Delta}}}
%\def\Thetaa{\acute{{\Theta}}}
%\def\Lambdaa{\acute{{\Lambda}}}
%\def\Pia{\acute{{\Pi}}}
%\def\Sigmaa{\acute{{\Sigma}}}
%\def\Upsilona{\acute{{\Upsilon}}}
%\def\Phia{\acute{{\Phi}}}
%\def\Psia{\acute{{\Psi}}}
%\def\Omegaa{\acute{{\Omega}}}
%
%
%%  check greeks
%\def\alphac{\check{{\alpha}}}
%\def\betac{\check{{\beta}}}
%\def\gammac{\check{{\gamma}}}
%\def\deltac{\check{{\delta}}}
%\def\epsilonc{\check{{\epsilon}}}
%\def\zetac{\check{{\zeta}}}
%\def\etac{\check{{\eta}}}
%\def\thetac{\check{{\theta}}}
%\def\iotac{\check{{\iota}}}
%\def\kappac{\check{{\kappa}}}
%\def\lambdac{\check{{\lambda}}}
%\def\muc{\check{{\mu}}}
%\def\nuc{\check{{\nu}}}
%\def\pic{\check{{\pi}}}
%\def\rhoc{\check{{\rho}}}
%\def\sigmac{\check{{\sigma}}}
%\def\tauc{\check{{\tau}}}
%\def\upsilonc{\check{{\upsilon}}}
%\def\phic{\check{{\phi}}}
%\def\chic{\check{{\chi}}}
%\def\psic{\check{{\psi}}}
%\def\omegac{\check{{\omega}}}
%\def\Gammac{\check{{\Gamma}}}
%\def\Deltac{\check{{\Delta}}}
%\def\Thetac{\check{{\Theta}}}
%\def\Lambdac{\check{{\Lambda}}}
%\def\Pic{\check{{\Pi}}}
%\def\Sigmac{\check{{\Sigma}}}
%\def\Upsilonc{\check{{\Upsilon}}}
%\def\Phic{\check{{\Phi}}}
%\def\Psic{\check{{\Psi}}}
%\def\Omegac{\check{{\Omega}}}
%
%
%
%%  dot greeks
%\def\alphad{\dot{{\alpha}}}
%\def\betad{\dot{{\beta}}}
%\def\gammad{\dot{{\gamma}}}
%\def\deltad{\dot{{\delta}}}
%\def\epsilond{\dot{{\epsilon}}}
%\def\zetad{\dot{{\zeta}}}
%\def\etad{\dot{{\eta}}}
%\def\thetad{\dot{{\theta}}}
%\def\iotad{\dot{{\iota}}}
%\def\kappad{\dot{{\kappa}}}
%\def\lambdad{\dot{{\lambda}}}
%\def\mud{\dot{{\mu}}}
%\def\nud{\dot{{\nu}}}
%\def\pid{\dot{{\pi}}}
%\def\rhod{\dot{{\rho}}}
%\def\sigmad{\dot{{\sigma}}}
%\def\taud{\dot{{\tau}}}
%\def\upsilond{\dot{{\upsilon}}}
%\def\phid{\dot{{\phi}}}
%\def\chid{\dot{{\chi}}}
%\def\psid{\dot{{\psi}}}
%\def\omegad{\dot{{\omega}}}
%\def\Gammad{\dot{{\Gamma}}}
%\def\Deltad{\dot{{\Delta}}}
%\def\Thetad{\dot{{\Theta}}}
%\def\Lambdad{\dot{{\Lambda}}}
%\def\Pid{\dot{{\Pi}}}
%\def\Sigmad{\dot{{\Sigma}}}
%\def\Upsilond{\dot{{\Upsilon}}}
%\def\Phid{\dot{{\Phi}}}
%\def\Psid{\dot{{\Psi}}}
%\def\Omegad{\dot{{\Omega}}}
%
%
%%  double dot greeks
%\def\alphadd{\ddot{{\alpha}}}
%\def\betadd{\ddot{{\beta}}}
%\def\gammadd{\ddot{{\gamma}}}
%\def\deltadd{\ddot{{\delta}}}
%\def\epsilondd{\ddot{{\epsilon}}}
%\def\zetadd{\ddot{{\zeta}}}
%\def\etadd{\ddot{{\eta}}}
%\def\thetadd{\ddot{{\theta}}}
%\def\iotadd{\ddot{{\iota}}}
%\def\kappadd{\ddot{{\kappa}}}
%\def\lambdadd{\ddot{{\lambda}}}
%\def\mudd{\ddot{{\mu}}}
%\def\nudd{\ddot{{\nu}}}
%\def\pidd{\ddot{{\pi}}}
%\def\rhodd{\ddot{{\rho}}}
%\def\sigmadd{\ddot{{\sigma}}}
%\def\taudd{\ddot{{\tau}}}
%\def\upsilondd{\ddot{{\upsilon}}}
%\def\phidd{\ddot{{\phi}}}
%\def\chidd{\ddot{{\chi}}}
%\def\psidd{\ddot{{\psi}}}
%\def\omegadd{\ddot{{\omega}}}
%\def\Gammadd{\ddot{{\Gamma}}}
%\def\Deltadd{\ddot{{\Delta}}}
%\def\Thetadd{\ddot{{\Theta}}}
%\def\Lambdadd{\ddot{{\Lambda}}}
%\def\Pidd{\ddot{{\Pi}}}
%\def\Sigmadd{\ddot{{\Sigma}}}
%\def\Upsilondd{\ddot{{\Upsilon}}}
%\def\Phidd{\ddot{{\Phi}}}
%\def\Psidd{\ddot{{\Psi}}}
%\def\Omegadd{\ddot{{\Omega}}}





==> tab/ablations.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Ours v0 & Frumpy \\
Ours v1 & Frobbly \\
\textbf{Ours} & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} %< \resizebox
\caption{
% 
\textbf{Ablations} -- our decisions are well justified.
% 
} % \caption
\label{tab:ablations}
\end{table}

==> tab/sota.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
% 
\textbf{State of the art} -- Glory to the bold numbers.
% 
} % \caption
\label{tab:sota}
\end{table}
